Coloring the Past: Neural Historical Buildings Reconstruction from Archival Photography

Historical buildings are a treasure and milestone of human cultural heritage. Reconstructing the 3D models of these building hold significant value. The rapid development of neural rendering methods makes it possible to recover the 3D shape only based on archival photographs. However, this task presents considerable challenges due to the limitations of such datasets. Historical photographs are often limited in number and the scenes in these photos might have altered over time. The radiometric quality of these images is also often sub-optimal. To address these challenges, we introduce an approach to reconstruct the geometry of historical buildings, employing volumetric rendering techniques. We leverage dense point clouds as a geometric prior and introduce a color appearance embedding loss to recover the color of the building given limited available color images. We aim for our work to spark increased interest and focus on preserving historical buildings. Thus, we also introduce a new historical dataset of the Hungarian National Theater, providing a new benchmark for the reconstruction method.

==> figure_tex/mesh_normal.tex <==
\begin{figure*}[ht]
\centering
\setlength{\tabcolsep}{2pt}
\newcolumntype{Y}{>{\centering\arraybackslash}p{0.22\linewidth}}
\begin{tabular}{lYYYY}
& Metashape~\cite{metashape2019} & NeusW~\cite{sun2022neuconw} & Neus-facto~\cite{Yu2022SDFStudio} & Ours \\
    \rotatebox{90}{Theater} & 
    \includegraphics[width=\linewidth]{imgs/comparison/theater/metashape_normal.png} &
    \includegraphics[width=\linewidth, clip, viewport=250 120 600 404]{imgs/comparison/theater/neusW_normal.png} & 
    \includegraphics[width=\linewidth, clip, viewport=250 120 600 404]{imgs/comparison/theater/facto_normal.png} & 
    \includegraphics[width=\linewidth, clip, viewport=250 120 600 404]{imgs/comparison/theater/ours_normal.png}  \\
      \rotatebox{90}{\small Observatory} & 
    \includegraphics[width=\linewidth]{imgs/comparison/observatory/metashape_normal_crop.png} & 
    \includegraphics[width=\linewidth, clip, viewport=100 0 800 452]{imgs/comparison/observatory/neusW_normal_crop.png} & 
    \includegraphics[width=\linewidth, clip, viewport=200 100 800 524]{imgs/comparison/observatory/facto_normal_crop.png} &
    \includegraphics[width=\linewidth, clip, viewport=100 200 800 707]{imgs/comparison/observatory/ours_normal_crop.png} \\
    \rotatebox{90}{Church} & 
    \includegraphics[width=\linewidth]{imgs/comparison/church/metashape_normal_crop.png} & 
    \includegraphics[width=\linewidth, clip, viewport=160 205 610 640]{imgs/comparison/church/neusW_normal_crop.png} & 
    \includegraphics[width=\linewidth, clip, viewport=160 205 610 640]{imgs/comparison/church/facto_normal_crop.png} &
    \includegraphics[width=\linewidth, clip, viewport=160 205 610 640]{imgs/comparison/church/ours_normal_crop.png}
    \\
    \rotatebox{90}{Hotel} & 
    \includegraphics[width=\linewidth, clip, viewport=100 0 750 300]{imgs/comparison/hotel/metashape_normal_crop.png} & 
     \includegraphics[width=\linewidth, clip, viewport=150 0 750 300]{imgs/comparison/hotel/neusW_normal_crop.png} & 
     \includegraphics[width=\linewidth, clip, viewport=150 0 750 300]{imgs/comparison/hotel/facto_normal_crop.png} &
     \includegraphics[width=\linewidth, clip, viewport=150 0 750 300]{imgs/comparison/hotel/ours_cut_normal_crop.png}
\end{tabular}
\caption{Normal map of the recovered geometry.}\label{fig:historical_results}
\end{figure*}

==> figure_tex/normal_results.tex <==

\begin{figure}[]
\centering
  \begin{tabular}{@{}rcccc@{}}
    & Theater & Observatory & Church & Hotel \\
    
    % \rotatebox{90}{Ground Truth} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/gt/theater/fortepan_59850.jpg} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/gt/observatory/1427.jpg} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/gt/church/A6_458.jpg} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/gt/hotel/2573.jpg} &
    % \\
    
    % \rotatebox{90}{NerfW} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/nerfw/theater_facade_static.png} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/nerfw/observatory_static.png} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/nerfw/square_static.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/nerfw/stockholm_static.png}  \\


    \rotatebox{90}{Metashape\cite{}} & 
    \includegraphics[width=.23\textwidth]{imgs/comparison/metashape/theater/fortepan_59850.jpg_normals.png} & 
    \includegraphics[width=.23\textwidth]{imgs/comparison/metashape/observatory/1427.jpg_normals.png} & 
    \includegraphics[width=.23\textwidth]{imgs/comparison/metashape/church/A6_458.jpg_normals.png} &
    \includegraphics[width=.23\textwidth]{imgs/comparison/metashape/hotel/2573.jpg_normals.png}  \\
    
    % \rotatebox{90}{Colmap} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/colmap/theater/fortepan_59850.jpg_normals.png} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/colmap/observatory/1427.jpg_normals.png} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/colmap/church/A6_458.jpg_normals.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/colmap/hotel/2573.jpg_normals.png}  \\

    % we can take this off as this is the baseline in other plots
    \rotatebox{90}{NeuS-Facto} & 
    \includegraphics[width=.23\textwidth]{imgs/sdf/1.png} &
    \includegraphics[width=.23\textwidth]{imgs/sdf/depth_1.png} &
    \includegraphics[width=.23\textwidth]{imgs/sdf/depth_1.png} &
    \includegraphics[width=.23\textwidth]{imgs/sdf/normal_1.png} \\

    % baseline
    \rotatebox{90}{NeuS-W2k} & 
    \includegraphics[width=.23\textwidth]{imgs/comparison/neusW-2k/theater/fortepan_59850.jpg_normals.png} &
    \includegraphics[width=.23\textwidth]{imgs/comparison/neusW-2k/observatory/1427.jpg_normals.png} &
    \includegraphics[width=.23\textwidth]{imgs/comparison/neusW-2k/church/A6_458.jpg_normals.png} &
    \includegraphics[width=.23\textwidth]{imgs/comparison/neusW-2k/hotel/2573.jpg_normals.png} \\ 
    
    % \rotatebox{90}{NeuS-W4k} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/neusW-4k/theater/fortepan_59850.jpg_normals.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/neusW-4k/observatory/1427.jpg_normals.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/neusW-4k/church/A6_458.jpg_normals.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/neusW-4k/hotel/2573.jpg_normals.png} \\    
    \rotatebox{90}{MonoSDF} & 
    \includegraphics[width=.23\textwidth]{imgs/comparison/monosdf_2k/theater/fortepan_59850.jpg_normals.png} &
    \includegraphics[width=.23\textwidth]{imgs/comparison/monosdf_2k/observatory/1427.jpg_normals.png} &
    \includegraphics[width=.23\textwidth]{imgs/comparison/monosdf_4k/church/A6_458.jpg_normals.png} &
    \includegraphics[width=.23\textwidth]{imgs/comparison/monosdf_4k/hotel/2573.jpg_normals.png} \\
    
    % \rotatebox{90}{Ours (dense} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/sfm_dense_0.1/theater/fortepan_59850.jpg_normals.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/sfm_dense_0.1/observatory/1427.jpg_normals.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/sfm_dense_0.1/church/A6_458.jpg_normals.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/sfm_dense_0.1/hotel/2573.jpg_normals.png} \\
    
    
    % \rotatebox{90}{Ours (sparse dense} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/sfm_sparse_dense_0.1/theater/fortepan_59850.jpg_normals.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/sfm_sparse_dense_0.1/observatory/1427.jpg_normals.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/sfm_sparse_dense_0.1/church/A6_458.jpg_normals.png} &
    % \includegraphics[width=.23\textwidth]{imgs/comparison/sfm_sparse_dense_0.1/hotel/2573.jpg_normals.png} \\
    
    \rotatebox{90}{Ours (color dense)} & 
    \includegraphics[width=.23\textwidth]{imgs/comparison/color_sfm_dense_0.1/theater/fortepan_59850.jpg_normals.png} &
    \includegraphics[width=.23\textwidth]{imgs/comparison/color_sfm_dense_0.1/observatory/1427.jpg_normals.png} &
    \includegraphics[width=.23\textwidth]{imgs/comparison/color_sfm_dense_0.1/church/A6_458.jpg_normals.png} &
    \includegraphics[width=.23\textwidth]{imgs/comparison/color_sfm_dense_0.1/hotel/2573.jpg_normals.png} \\
    
    
  \end{tabular}
  \caption{Comparison to other methods (normal)}
  \label{fig:comparison_other_methods}


  Our method results in a more geometrically accurate models with finer details an retains thin structures. Howerever it also has some artifacts originating from imprecise Sfm point cloud.
  Color loss causes bigger holes at windows because the color of the interior significantly changes which has a smaller impact in grayscale.
\end{figure}

==> figure_tex/novel_view.tex <==
\begin{figure}[]
\centering
  \begin{tabular}{cccccc}
    & BG 90 & Theater & Church & Hotel  & Observatory \\
    
    \rotatebox{90}{Ground Truth/Reference Foto} & 
    \includegraphics[width=.15\textwidth]{imgs/color/brandenburg_gate_gt_gray.png} &
    \includegraphics[width=.15\textwidth]{imgs/comparison/gt/theater/fortepan_31611.jpg} &
    \includegraphics[width=.20\textwidth]{imgs/comparison/gt/church/A6_458.jpg} &
    \includegraphics[width=.20\textwidth]{imgs/comparison/gt/hotel/2573.jpg} &
    \includegraphics[width=.20\textwidth]{imgs/comparison/gt/observatory/1427.jpg} 
    \\
    
    % \rotatebox{90}{NerfW} & 
    % \includegraphics[width=.15\textwidth]{imgs/comparison/nerfw/brandenburg_gate_historic_90.png} &
    % \includegraphics[width=.20\textwidth]{imgs/comparison/nerfw/theater_facade.jpg} & % change to clean this is a placeholder
    % \includegraphics[width=.20\textwidth]{imgs/comparison/nerfw/st_michael_church.jpg} &
    % \includegraphics[width=.20\textwidth]{imgs/comparison/nerfw/hotel_static.png} &
    % \includegraphics[width=.20\textwidth]{imgs/comparison/nerfw/observatory_.jpg}  \\
    
    
    \rotatebox{90}{Baseline} & 
    \includegraphics[width=.15\textwidth]{imgs/color/neusw/brandenburg_gate_90-baseline_2k.png} &
    \includegraphics[width=.20\textwidth]{imgs/color/neusw/theater_clean-baseline_2k.png} &
    \includegraphics[width=.20\textwidth]{imgs/color/neusw/church-baseline_2k.png} &
    \includegraphics[width=.20\textwidth]{imgs/color/neusw/hotel-baseline_2k.png} &
    \includegraphics[width=.20\textwidth]{imgs/color/neusw/observatory-baseline_2k.png}  \\
    
    \rotatebox{90}{Color (Ours)} & 
    \includegraphics[width=.15\textwidth]{imgs/color/neusw/brandenburg_gate_90-color_sfm_dense_0.1_2k.png} &
    \includegraphics[width=.20\textwidth]{imgs/color/neusw/theater_clean-color_sfm_dense_0.1_2k.png} &
    \includegraphics[width=.20\textwidth]{imgs/color/neusw/church-color_sfm_dense_0.1_2k.png} &
    \includegraphics[width=.20\textwidth]{imgs/color/neusw/hotel-color_sfm_dense_0.1_2k.png} &
    \includegraphics[width=.20\textwidth]{imgs/color/neusw/observatory-color_sfm_dense_0.1_2k.png}  \\
    
  \end{tabular}
  \caption{Novel view synthesis: color comparirison NEUS-W base}
  \label{fig:color_comparison}
\end{figure}

==> figure_tex/old_figure.tex <==
\begin{figure}[]
\centering
  \begin{tabular}{@{}rcccc@{}}
    & theater & observatory & church & hotel \\
    
    % \rotatebox{90}{GT} & 
    % \includegraphics[width=.23\textwidth]{imgs/comparison/gt/theater/fortepan_59850.jpg} &
    % \\
    % \rotatebox{90}{Baseline} & 
    % \includegraphics[width=.23\textwidth]{imgs/ablation/theater/baseline_fortepan_59850.jpg_color.png} &
    % \\
    
    \rotatebox{90}{Color} & 
    \includegraphics[width=.23\textwidth]{imgs/ablation/theater/color_fortepan_59850.jpg_color.png} 
        \\
    
    \rotatebox{90}{Sparse} & 
    \includegraphics[width=.23\textwidth]{imgs/ablation/theater/sparse_fortepan_59850.jpg_color.png} \\
    
    \rotatebox{90}{Dense} & 
    \includegraphics[width=.23\textwidth]{imgs/ablation/theater/dense_fortepan_59850.jpg_color.png} \\    
    
    \rotatebox{90}{Color + Dense + (?Sparse)} & 
    \includegraphics[width=.23\textwidth]{imgs/sdf/normal_2.png} \\
    
    
  \end{tabular}
  \caption{Ablation study on historic
  rows: gt, (baseline neus-facto), color loss, sparse, dense,  all (dense+sparse+color)
  columns: brandenburg, brandernburg subsets 100/40, challenging side of theater}
  \label{fig:ablation_historic}
\end{figure}
